A Hierarchical Architecture for Optimal Unit Commitment and Control of an Ensemble of Steam Generators

A hierarchical architecture for the optimal management of an ensemble of steam generators is presented. The subsystems are coordinated by a multilayer scheme for jointly sustaining a common load. The high level optimizes the load allocation and the generator schedule, considering activation dynamics by a hybrid model. At the medium level, a robust tube-based model predictive control (MPC) tracks a time-varying demand using a centralized--but aggregate--model, whose order does not scale with the number of subsystems. A nonlinear optimization, at medium level, addresses MPC infeasibility due to abrupt changes of ensemble configuration. Low-level decentralized controllers stabilize the generators. This control scheme enables the dynamical modification of the ensemble configuration and plug and play operations. Simulations demonstrate the approach potentialities.

==> Authors_bio/bio_with_photos.tex <==
\vskip -3\baselineskip plus -1fil
%\begin{IEEEbiographynophoto}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{spine.jpg}}]{Stefano Spinelli} received the master's degree in aeronautical engineering and the Ph.D. degree in Information Technology from the Politecnico di Milano, in 2012 and 2021, respectively. Since 2013 he is a researcher at Consiglio Nazionale delle Ricerche at the Istituto di Sistemi e 	Tecnologie Industriali Intelligenti per il Manifatturiero Avanzato. His research interests include optimization and control of large-scale systems, and energy-aware scheduling of industrial processes for demand response.
\end{IEEEbiography}
%\end{IEEEbiographynophoto}%
\vskip -3\baselineskip plus -1fil
%\begin{IEEEbiographynophoto}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{farin.jpg}}]{Marcello Farina} received the master’s degree in electronic engineering and the Ph.D. degree in information engineering from the Politecnico di Milano, Milan, Italy, in 2003 and 2007, respectively. He was Visiting Student with the Institute for Systems Theory and Automatic Control, Stuttgart, Germany, in 2005. He is currently an Associate Professor with the Dipartimento di Elettronica, Informazione, e Bioingegneria, Politecnico di Milano. His current research interests include distributed, hierarchical and decentralized state estimation and control, stochastic model predictive control, and applications, including mobile robots, sensor networks, and energy supply systems.	
\end{IEEEbiography}
%\end{IEEEbiographynophoto}%
\vskip -3\baselineskip plus -1fil
%\begin{IEEEbiographynophoto}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{balla.png}}]{Andrea Ballarino} received the master’s degree in Computer Science and Engineering - with specialisation in  robotics and industrial automation - in 2001, from the Politecnico di Milano. He is currently responsible of 2MaCS - Machine and Manufacturing Control System Group within the Istituto di Sistemi e Tecnologie Industriali Intelligenti per il Manifatturiero Avanzato of Consiglio Nazionale delle Ricerche. His research interests focus on methodologies and tools for distributed automation systems design and development, adaptive and sustainable automation systems, model predictive control and real time process optimization, hybrid control systems. 
\end{IEEEbiography}
%\end{IEEEbiographynophoto}%
